Communication- and Computation-Efficient Distributed Submodular Optimization in Robot Mesh Networks

We provide a communication- and computation-efficient method for distributed submodular optimization in robot mesh networks. Submodularity is a property of diminishing returns that arises in active information gathering such as mapping, surveillance, and target tracking. Our method, Resource-Aware distributed Greedy (RAG), introduces a new distributed optimization paradigm that enables scalable and near-optimal action coordination. To this end, RAG requires each robot to make decisions based only on information received from and about their neighbors. In contrast, the current paradigms allow the relay of information about all robots across the network. As a result, RAG's decision-time scales linearly with the network size, while state-of-the-art near-optimal submodular optimization algorithms scale cubically. We also characterize how the designed mesh-network topology affects RAG's approximation performance. Our analysis implies that sparser networks favor scalability without proportionally compromising approximation performance: while RAG's decision time scales linearly with network size, the gain in approximation performance scales sublinearly. We demonstrate RAG's performance in simulated scenarios of area detection with up to 45 robots, simulating realistic robot-to-robot (r2r) communication speeds such as the 0.25 Mbps speed of the Digi XBee 3 Zigbee 3.0. In the simulations, RAG enables real-time planning, up to three orders of magnitude faster than competitive near-optimal algorithms, while also achieving superior mean coverage performance. To enable the simulations, we extend the high-fidelity and photo-realistic simulator AirSim by integrating a scalable collaborative autonomy pipeline to tens of robots and simulating r2r communication delays. Our code is available at https://github.com/UM-iRaL/Resource-Aware-Coordination-AirSim.

==> preamble_packages.tex <==
%!TEX root = main.tex
\newcommand{\ie}{\emph{i.e.},\xspace}
\newcommand{\eg}{\emph{e.g.},\xspace}
% \newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\myin}{\, \in \,}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}

\newcommand{\sg}{\scenario{SG}}
\newcommand{\banalg}{\scenario{BSGC}}
% \newcommand{\sgd}{{\scenario{\widehat{SG}}}}
% \newcommand{\sgh}{\text{\scenario{SG}-\scenario{Heuristic}}}
\newcommand{\sgh}{{\fontsize{9}{9}\selectfont\sf SG\text{-}Heuristic}}
\newcommand{\dfs}{\scenario{DFS-SG}}



\newcommand{\myprob}{Problem~\ref{pr:main}\xspace}
\newcommand{\CPP}{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\tiny\bf +}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\tiny\bf +}}
\def\CC{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\tiny\bf ++}}}
\newcommand{\MATLAB}{\textsc{MATLAB}}


\newcommand{\myParagraph}[1]{{\bf #1.}\xspace}


%text shortcuts
\newcommand{\changed}[1]{{\color{myblue}{#1}}}
\newcommand{\review}[2]{{#2}}
\newcommand{\validated}[2]{{#2}}
\newcommand{\subjectTo}{\rm{s.t.}}

\newcommand{\inneigh}{\calN^-}
\newcommand{\outneigh}{\calN^+}
\renewcommand{\opt}{\scenario{OPT}}
\newcommand{\single}{s}
\newcommand{\robset}{\calN}
\newcommand{\selset}{\calN}
\newcommand{\curv}{\kappa}
\newcommand{\ourcurv}{\scenario{coin}}
\newcommand{\ourcurvname}{Independence from Non-Neighbors }
\newcommand{\ouragent}{\mathcal{N}}
% \newcommand{\alg}{\textsc{AnaCoNDa}\xspace}
\newcommand{\alg}{\scenario{Anaconda}}
\newcommand{\actionsel}{\scenario{ActionCoordination}}
\newcommand{\neighborsel}{\scenario{NeighborSelection}}
\newcommand{\oursol}{\calA^{\alg}}
\newcommand{\numl}{\scenario{length}_\#}
\newcommand{\el}{\scenario{length}_a}
\newcommand{\rob}{j}
\newcommand{\elem}{v}

\newcommand{\fsf}[1]{\scenario{FSF$^{\star}|_{#1}$}}
\newcommand{\expsix}[1]{\scenario{EXP3$^{\star}$-SIX$|_{#1}$}}
\newcommand{\solosg}{\calA^{\onalg}}
\newcommand{\solbsg}{\calA^{\banalg}}
\newcommand{\distfsf}{p}
\newcommand{\onalg}{\scenario{OSG}}
\newcommand{\solopt}{\calA^{\opt}}
\newcommand{\allfsf}{\mathcal{K}}
% \newcommand{\expsix}{\scenario{EXP3$^\star$-SIX}}
\newcommand{\distbanalg}{\scenario{DBG}}


\newcommand{\obsenv}{E_t^{obs}}
\newcommand{\env}{E_t}

\newcommand{\AReg}{\operatorname{A-Reg}_{T}}
\newcommand{\NReg}{\operatorname{N-Reg}_{\{a_t\}_{t\in [T]}}}
\newcommand{\expix}[1]{\scenario{EXP3-IX$|_{#1}$}}
\newcommand{\mwu}[1]{\scenario{MWU$|_{#1}$}}
\newcommand{\bsg}[1]{\scenario{BSGC$|_{#1}$}}
\newcommand{\expthreeix}{\scenario{EXP3-IX}}
\newcommand{\smi}[2]{I_{f,\,t}({#1};\,{#2})}

